Learning to Learn in a Semi-Supervised Fashion

To address semi-supervised learning from both labeled and unlabeled data, we present a novel meta-learning scheme. We particularly consider that labeled and unlabeled data share disjoint ground truth label sets, which can be seen tasks like in person re-identification or image retrieval. Our learning scheme exploits the idea of leveraging information from labeled to unlabeled data. Instead of fitting the associated class-wise similarity scores as most meta-learning algorithms do, we propose to derive semantics-oriented similarity representations from labeled data, and transfer such representation to unlabeled ones. Thus, our strategy can be viewed as a self-supervised learning scheme, which can be applied to fully supervised learning tasks for improved performance. Our experiments on various tasks and settings confirm the effectiveness of our proposed approach and its superiority over the state-of-the-art methods.

==> figure/fig_sensitivity.tex <==
\begin{figure}[!t]
  \begin{center}
    \includegraphics[width=\linewidth]{figure/images/sensitivity.pdf}
    \caption{\textbf{Sensitivity analysis of the similarity threshold $\psi$.} The performance of our approach remains stable when the similarity threshold $\psi$ is within a reasonable range.}
    \label{fig:sensitivity}
  \end{center}
\end{figure}
